An example of a weakly mixing BV vector field which is not strongly mixing

We give an example of a weakly mixing vector field $b\in L^\infty([0,1],\text{BV}(\mathbb{T}^2))$ which is not strongly mixing. The example is based on a work of Chacon who constructed a weakly mixing automorphism which is not strongly mixing on $([0,1],\mathcal{B}([0,1]),|\cdot|)$, where $\mathcal{B}([0,1])$ are the Borel subsets of $[0,1]$ and $|\cdot|$ is the one-dimensional Lebesgue measure.

==> appunti2.tex <==
 \noindent Let us consider the two dimensional torus $\T^2$ as the unit square $Q_1=Q_{1,1}=[0,1]^2$ with the canonical identification of boundaries. Using the notation with configurations (see Section \ref{subS_rows_columns}) we say that $Q_1$ can be identified with any configuration $\gamma_1\in\mathcal{C}(1)$: for simplicity we choose $\gamma_1=0$. We divide the square $Q_1=Q_{1,1}$ into four identical subsquares each one of side $\frac{1}{2}$, more precisely: $Q_{1,1}=Q_{1,1}(1)\cup Q_{1,1}(2)\cup Q_{1,1}(4)\cup R_1$ where $Q_{1,1}=[0,\frac{1}{2}]^2$, $Q_{1,1}(2)=[\frac{1}{2},1]\times[0,\frac{1}{2}]$ and $Q_{1,1}(3)=[0,\frac{1}{2}]\times [\frac{1}{2},1]$. We define $U_1$ on subsquares in such a way that 
 \begin{equation}
     U_1(Q_{0,1}(1))=Q_{0,1}(2), \quad U_{1}(Q_{0,1}(2))=Q_{0,1}(4)
 \end{equation}
 and $U_1$ is measure-preserving and invertible on $Q_{0,1}$. More precisely, we want $U_1$ piecewise affine on $Q_{0,1}(1),Q_{0,1}(2)$, that is  (definizione a.e. ? vedi Zlatos)
 \begin{equation}
     U_1(x)=\begin{cases}
     x+(\frac{1}{2},0) \quad\text{if}\quad x\in Q_{0,1}(1), \\
     x+(-\frac{1}{2},\frac{1}{2}) \quad\text{if}\quad x\in Q_{0,1}(2),\\
     x+(0,-\frac{1}{2}) \quad\text{if}\quad x\in Q_{0,1}(4), \\
     x \quad\text{otherwise}.
     \end{cases}
 \end{equation}
 
 \noindent We put $h_1=3$ and we rename the subsquares $Q_{0,i}$ as $Q_{1,1}=Q_{0,1}(1), Q_{1,2}=Q_{0,1}(2), Q_{1,3}=Q_{0,1}(4)$.
 We divide each of the subsquares $Q_{1,i}$ with $i\in\lbrace{1,2,3}\rbrace$ into $4$ subsquares: $Q_{1,i}=Q_{1,i}(1)\cup Q_{i,1}(2)\cup Q_{i,1}(3)\cup Q_{1,i}(4)$ and we divide also $R_1=R_{1}(1)\cup R_{1}(2)\cup R_{1}(4)\cup R_2$ (see Figure \ref{twodsub}) into $4$ subsquares. 
 \begin{figure}
     \centering
     \includegraphics[scale=0.5]{twodsubdivision.png}
     \caption{Subdivisions of the unit torus}
     \label{twodsub}
 \end{figure}
 We define the map $U_2$ in the following way
\begin{equation}
    U_2(x)=\begin{cases}
    U_1(x) \quad\text{if}\quad x\in Q_{1,1}\cup Q_{1,2}, \\
    x +(\frac{1}{4},-\frac{1}{2}) \quad\text{if}\quad x\in Q_{1,3}(1), \\
    x +(-\frac{1}{4},0) \quad\text{if}\quad x\in Q_{1,3}(2) ,\\
    x +(\frac{1}{2},-\frac{1}{4}) \quad\text{if}\quad x\in Q_{1,3}(3), \\
    x +(\frac{1}{2},0) \quad\text{if}\quad x\in Q_{1,3}(4), \\
     x +(-\frac{1}{4},-\frac{1}{4})  \quad\text{if}\quad x\in R_1(1), \\
    x +(-\frac{3}{4},-\frac{1}{4}) \quad\text{if}\quad x\in R_1(2), \\
    x +(-\frac{1}{2},-\frac{3}{4}) \quad\text{if}\quad x\in R_1(4), \\
     x \quad\text{otherwise}.
    \end{cases}
\end{equation}
 We put $h_2=4h_1+3=15$ and we rename the squares as $Q_{1,i}(j)=Q_{2, j+(i-1)2^2}$ if $i< h_1+1$ and $R_1(1)=Q_{2,13}, R_1(2)=Q_{2,14}, R_1(4)= Q_{2,15}$. \\
 
\noindent The inductive step is the following: at the $n$-th step we have $Q_{n,1},\dots Q_{n,h_n}$ subsquares of area $\frac{1}{(h_n+1)}$. We call $l_n=\sqrt{h_n+1}$ We divide each subsquare into 4 identical subsquares: $Q_{n,i}=Q_{n,i}(1)\cup Q_{n,i}(2)\cup Q_{n,i}(3)\cup Q_{n,i}(4)$ and we divide $R_{n-1}=R_{n-1}(1)\cup R_{n-1}(2)\cup R_{n-1}(4)\cup R_n$. We define the map $U_{n+1}$ in the following way:
\begin{equation}
    U_{n+1}(x)=\begin{cases}
    U_n(x) \quad\text{if}\quad x\in Q_{n,1}\cup\dots\cup Q_{1,h_{n-1}} \\
      x +(\frac{l_n-3}{l_n},-\frac{l_n-2}{l_n}) \quad\text{if}\quad x\in Q_{n,h_n}(1) \\
    x +(-\frac{l_n-3}{l_n},0) \quad\text{if}\quad x\in Q_{n,h_n}(2) \\
    x +(\frac{l_n-2}{l_n},-\frac{l_n-3}{l_n}) \quad\text{if}\quad x\in Q_{n,h_n}(3) \\
    x +(\frac{l_n-2}{l_n},0) \quad\text{if}\quad x\in Q_{n,h_n}(4) \\
     x +(-\frac{l_n-3}{l_n},-\frac{l_n-3}{l_n})  \quad\text{if}\quad x\in R_n(1) \\
    x +(-\frac{l_n-1}{l_n},-\frac{l_n-3}{l_n}) \quad\text{if}\quad x\in R_n(2) \\
    x +(-\frac{l_n-2}{l_n},-\frac{l_n-1}{l_n}) \quad\text{if}\quad x\in R_n(4) \\
    x\quad\text{otherwise}.
    \end{cases}
    \end{equation}
 We put $h_{n+1}=4h_n+3$ and we rename the squares as $Q_{n,i}(j)=Q_{n+1, j+(i-1)2^2}$ if $i< h_n+1$ and $R_{n-1}(1)=Q_{n,(h_n+1)2^2}, R_{n-1}(2)=Q_{n,(h_n+2)2^2}, R_{n-1}(4)= Q_{n,(h_n+3)2^2}$, $R_{n-1}(3)=R_n$. 
 
 \begin{remark}\label{configurazione di riferimento}
In terms of configurations 
\begin{equation}
U_2\left(\begin{matrix}
12 & 11 & 15 & 0 \\ 9 & 10 & 13 & 14 \\ 4 & 3 & 8 & 7 \\ 1 & 2 & 5 & 6
\end{matrix}\right)=\left(\begin{matrix}
8 & 7 & 12 & 0 \\ 5 & 6 & 10 & 11 \\ 14 & 13 & 4 & 3 \\ 15 & 9 & 1 & 2
\end{matrix}\right).
\end{equation}
\end{remark}
 
 
 \begin{proposition}\label{prop:wm:not:sm}
 The map $U$ is a weakly mixing automorphism but it is not strongly mixing.
 \end{proposition}
 \begin{proof}
 The idea of the proof is the same of Chacon. Indeed: take for example a subsquare $Q=Q_{n,i}$ then one can easily check that, for $k\geq n-1$
 \begin{equation}
     |U^{h_{k}+1}(Q)\cap Q|\geq \frac{1}{2} |Q|.
 \end{equation}
 While $U$ is weakly mixing. We first observe that $U$ is measure-preserving and ergodic (come si dimostra?). By Theorem \ref{mixing theorem} we have to prove that if $f\in\L^2[0,1]$ is an eigenfunction of $\mathcal{U}_U$ of eigenvalue $\lambda$, with $|\lambda|=1$, then $f=c$ for some constant $c$. By Lemma $2$ of \cite{Ergodic:theory} (chapter 1, pag 14), we need only to prove that $\lambda=1$. Since $f$ is non-zero on a set of positive measure, for every $\epsilon>0$ there exists a constant $k$ such that the set
$$ A=\lbrace x: |f(x)-k|<\epsilon\rbrace $$ has positive measure. By Lebesgue Density Theorem there exists some subsquare $Q=Q_{n,i}$ such that 
\begin{equation}\label{density}
    \frac{|Q\cap A|}{|Q|}> \frac{7}{8}.
\end{equation}
As in the previous computations, since $Q=Q(1)\cup Q(2)\cup Q(3)\cup Q(4)$ and
$U^{h_n}(Q(1))=Q(2)$, $S^{2h_n+1}(Q(1))=Q(3)$, using that $U$ is measure-preserving and \ref{density} we obtain that there exists a point $x\in A\cap Q$ such that $U^{h_n}(x)\in A\cap Q$, and that there exists $y\in A\cap Q$ such that $U^{2h_n+1}(y)\in A\cap Q$. Indeed, by \eqref{density} we have that $|Q(2)\cap A|>\frac{1}{8}|Q|$ and since
$$ |Q(2)\cap U^{h_n}(A)|>\frac{1}{8}|Q| $$ we have that $$ |(Q\cap A)\cap U^{h_n}(Q\cap A)|>0.$$ An analogous argument proves that $$ |(Q\cap A)\cap U^{2h_n+1}(Q\cap A)|>0.$$
Therefore
\begin{equation}
    |f(x)-k|<\epsilon, \quad |\lambda^{h_n}f(x)-k|<\epsilon, \quad |f(y)-k|<\epsilon, \quad
    |\lambda^{2h_n+1}f(y)-k|<\epsilon.
\end{equation}
So we have that, by the previous equations, that
\begin{equation*}
    \lambda= \frac{k+\delta_2}{k+\delta_1}, \quad \lambda^{2h_n+1}=\frac{k+\delta_4}{k+\delta_3}
\end{equation*}
with $|\delta_i|<\epsilon$ for every $i$. That is
\begin{equation}
    \lambda=\frac{(k+\delta_4)(k+\delta_1)^2}{(k+\delta_3)(k+\delta_2)^2},
\end{equation}
and since this hold for every $\epsilon>0$, we conclude that $\lambda=1$. 
 \end{proof}
 
 \noindent The maps $U_n$ can be decomposed into simple movements, using the terminology of configurations. This will allow us to construct a family $\lbrace b_n\rbrace $ of divergence-free $\BV$ vector field each one associated with $\lbrace U_n\rbrace$.  \\
 
 \noindent
 For simplicity, let us fix the step $n\in\N$ and some configuration $\gamma\in\mathcal{C}_n$. Then we have the following
 \begin{proposition}\label{movements_first construction}
 \begin{equation}
     U_n(\gamma)=s^2_c(2)\circ s^2_c(1)\circ R^{-}_{2,1}\circ o (1,n-2)\circ scambio ((1,n-2),(1,(n-1))\circ s^2_r(2)\circ R^+_{2,n-3}\circ s^2_r(3)\circ\dots\circ s^2_r(n)(\gamma).
 \end{equation}
 \end{proposition}
 \begin{remark}The interested reader can observe that $\forall k$ the map $U_k$ is a cyclic permutation of subsquares of same area (see \cite{Bianchini_Zizza_residuality} for the definitions). This observation is in the spirit of the result proved by Halmos in \cite{Halmos:weak:mix} that states that weakly mixing automorphisms are a residual $G_\delta$-set in $G(\T^2)$ with the $L^1$ topology. In \cite{Bianchini_Zizza_residuality} a key ingredient for the proof of Halmos result for vector fields (that applies to automorphisms as a corollary) was to perturb any possible cyclic permutation in order to get a strongly mixing vector field (and so weakly mixing). The fundamental idea is that we can produce either weakly mixing automorphisms or vector fields simply perturbing cyclic permutations. In this paper we are doing a different thing: we fix a specific cyclic permutation and we perturb it in order to have a weakly mixing automorphism. An open question would be to generalize Chacon's construction to any cyclic permutation in order to recover the same results obtained in \cite{Halmos:weak:mix} and \cite{Bianchini_Zizza_residuality}. \end{remark}
\subsection{Second construction}\label{subS_product}
The second construction exploits Theorem \ref{product}: once we know that an automorphism $T$ is weakly mixing, then the product map $T\times T$ is weakly mixing.   
Here, the price to pay is the proof that this new map is weakly mixing but not strongly mixing, while for the product map (that we will describe in the next section) this result is given for free by Theorem \ref{product}.
{\color{red} forse va introdotto uno spazio di configurazioni. Posso anche dire che questa costruzione è più naturale sul toro data la presenza degli shift, mentre la seconda costruzione è più naturale sul quadrato.}


\noindent
Finally we define $S_k=T_k\times T_k$ where $\lbrace T_k\rbrace$ is the family \ref{chacon limit} and $S=\lim_{k\to\infty}S_k=T\times T$, where $T$ is the Canonical Chacon's map. By Theorem \ref{product} we know that $S$ is weakly mixing. The map $S$ is not strongly mixing. The proof of this fact is a direct consequence of Fubini Theorem and of \eqref{eq_3_chacon1}. \\

\noindent We show now that each $S_k$ can be decomposed into a fixed number (not depending on $k$) of horizontal and vertical movements (as a two dimensional Rubik cube), each one arising as the action of a $BV$ divergence-free vector field. 
We start with $S_1$ to fix the notation and the notion of movements. We recall that by the previous analysis the map $T_1$ can be written as
\begin{equation*}
    T_1\llcorner_{[0,1]\setminus R_1}=\left(\begin{matrix}I_{0,1}(1) & I_{0,1}(2) & I_{0,1}(3) & S_0 \\ I_{0,1}(2) & S_0 & I_{0,1}(1) & I_{0,1}(3)\end{matrix}\right).
\end{equation*}
For simplicity, if we associate $I_{0,1}(j)\rightarrow j$ and $S_0\rightarrow 4$ we write it as
\begin{equation}\label{notation_permutation}
    T_1\llcorner_{[0,1]\setminus R_1}=\left(\begin{matrix}1 & 2 & 3 & 4 \\ 2 & 4 & 1 & 3\end{matrix}\right).
\end{equation}
We represent the action of the map $S_1$ in the following matrix form, where the couples $\lbrace i,j\rbrace$,  $i,j\in\lbrace{1,2,3,4}\rbrace$ where $i,j$ represent respectively the row and the column index, denote the subsquares of $\mathbb{T}^2$. Finally, $c_s$ and $c_f$ are the \emph{starting configuration} and the \emph{final configuration}: 
\begin{equation}\label{configurations}
    c_s=\left(\begin{matrix}4,1 & 4,2 & 4,3 & 4,4 \\ 3,1 & 3,2 & 3,3 & 3,4 \\ 2,1 & 2,2 & 2,3 & 2,4 \\ 1,1 & 1,2 & 1,3 & 1,4
    \end{matrix}\right)\stackrel{S_1}{\longrightarrow}  c_f=\left(\begin{matrix}2,3 & 2,1 & 2,4 & 2,2 \\ 4,3 & 4,1 & 4,4 & 4,2 \\ 1,3 & 1,1 & 1,4 & 1,2 \\ 3,3 & 3,1 & 3,4 & 3,2
    \end{matrix}\right)
\end{equation}
For example, $(1,1)$ denotes the subsquare $I_{0,1}^2=[0,\frac{2}{9}]^2$, therefore the action of the map $S_1$ is $S_1(1,1)=(T_1(1),T_1(1))=(2,2)=I_{0,1}(2)^2=[\frac{2}{9},\frac{4}{9}]$, that is the subsquare represented by $(1,1)$ is sent in the position of the subsquare $(2,2)$. One can easily observe that  each row is sent into another row, with permuted column indexes (ex. the row $(\begin{matrix}2,1 & 2,2 & 2,3 & 2,4\end{matrix})$ is sent into the row $(\begin{matrix} 4,2 & 4,4 & 4,1 & 4,3\end{matrix})$). The same for columns: each column is sent into another column with permuted row indexes. \\

\noindent
Given the starting configuration $c_s$ and the final configuration $c_f$ \ref{configurations} we describe the movements allowed to pass from $c_s\rightarrow c_f$.
Then we have
\begin{equation}\label{eq_movements_1}
     \gamma_f=(\rho_c(4)\circ\rho_c(1)\circ e_c(1,2)\circ s^3_c\circ e_c(1,2))\circ(\rho_r(4)\circ\rho_r(1)\circ e_r(1,2)\circ s^3_r\circ e_r(1,2))(\gamma_s).
\end{equation}
See in the appendix the proof of this fact. 
\begin{proposition}
Let us fix $n\in\N$ and let us consider the map $S_n$. Let $\gamma_s,\gamma_f$ be the starting and final configurations for $S_n$. Then
\begin{equation}\label{eq_movements}
    \gamma_f=(\rho_c(h_n)\circ\rho_c(1)\circ e_c(1,2)\circ s^3_c\circ e_c(h_{n}-3,h_n-2))\circ(\rho_r(h_n)\circ\rho_r(1)\circ e_r(1,2)\circ s^3_r\circ e_r(h_{n}-3,h_{n}-2))(\gamma_s)
\end{equation}
\begin{remark}
We observe that the \eqref{eq_movements} is consistent with \eqref{eq_movements_1} since $h_1=4$.
\end{remark}
\begin{proof}
We write the map $T_n$ as a permutation according to the notation \eqref{notation_permutation} (controlla se deve essere $h_n$ o $h_{n+1}$, la notazione delle configurazioni non va bene!!).
\begin{equation}\label{notation_permutations_n}
    T_n\llcorner_{[0,1]\setminus R_n}=\left(\begin{matrix}1 & 2 & 3 & \dots & i & \dots & h_{n}-3 & h_n-2 & h_n-1 & h_n \\ 4 & 5 & 6  & \dots & i+3 & \dots & 2  & h_n & 1 & 3  \end{matrix}\right).
\end{equation}
The starting configuration $\gamma_s$ for $S_n$ is $\gamma_s=(r(1),r(2),\dots,r(h_n))$, while the final one is $\gamma_f=(r(h_n-1), r(h_n-3), r(h_n), r(1), r(2),\dots, r(h_n-4), r(h_n-2))$, and the same if we write the configuration by columns. If we apply $(\rho_r(h_n)\circ\rho_r(1)\circ e_r(1,2)\circ s^3_r\circ e_r(h_{n}-3,h_{n}-2))$ to $\gamma_s$ we find
\begin{itemize}
\item
$e_r(h_{n}-3,h_{n}-2)(r(1),r(2),\dots,r(h_n))=(r(1),r(2),\dots,r(h_n-4), \bar{r}(h_n-2), \bar{r}(h_n-3), r(h_n-1), r(h_n))$,
    \item
    $s^3_r(r(1),r(2),\dots,r(h_n-4), \bar{r}(h_n-2), \bar{r}(h_n-3), r(h_n-1), r(h_n))= (\bar{r}(h_n-3), r(h_n-1), r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))$,
    \item $e_r(1,2)(\bar{r}(h_n-3), r(h_n-1), r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))=(\bar{r}(h_n-1),r(h_n-3),r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))$,
    \item $\rho_r(h_n)\circ\rho_r(1)(\bar{r}(h_n-1),r(h_n-3),r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))=(r(h_n-1),r(h_n-3),r(h_n),r(1),r(2),\dots)=\gamma_m$.
\end{itemize}
After this first set of movements we have the rows in the correct position, while the columns are ordered as $(c(1),c(2),\dots, c(h_n))$. This set of movements (horizontal/vertical ones) does not change the order of columns, as the second set of movements doesn't change the order of rows (questo è importante ma devo scriverlo in modo più esplicito). So applying the second set of movements to $\gamma_m$ since the order of rows does not change, while for columns we have the correct new order we finally get $\gamma_f$. Sono d'accordo che sia detto abbastanza a cazzo.
\end{proof}
 \end{proposition}
 \noindent The previous proposition shows that the number of movements to recover the final configuration of each map $S_n$ from the starting one is fixed: this result allows us to construct vector fields associated to each $S_n$. Anche le $S_n$ sono cicliche? da chiarirtelo.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Second construction}\label{subS_product}
Let us consider the Canonical chacon's map $T$ defined in Section \ref{Ss:chacon} on the unit interval $[0,1]$. As told in the introduction, we will produce this example on the unit square $[0,1]^2$ instead of the torus because we can give better compactness estimates on the vector fields (see Section \ref{Ss:second:estimates}. By Theorem \ref{product}, since $T$ is weakly mixing, then the product map $T\times T$ is weakly mixing on $[0,1]^2$.
Here, the price to pay is the proof that this new map is not strongly mixing, while for the previous case it followed by the same considerations of Chacon's proof \cite{Weaklymixingnotstrongly}.
\begin{proposition}
The automorphism $T\times T$ is not strongly mixing.
\end{proposition}
\begin{proof}
The proof is an easy consequence of the Fubini theorem. By contradiction, assume that $T\times T$ is strongly mixing, then
\begin{equation*}
    \lim_{n\to\infty}|(T\times T)^{-n}(A)\cap B|=|A||B|, \quad\forall A,B\in\mathcal{B}([0,1]^2).
\end{equation*}
Take $A=A'\times [0,1]$, $B=B'\times[0,1]$, $A',B'\in\mathcal{B}([0,1])$. Then we have
\begin{equation*}
    |(T\times T)^{-n}(A)\cap B|=|(T^{-n}(A')\cap B)\times [0,1]|=|(T^{-n}(A')\cap B)|,
\end{equation*}
where the last equality follows by Fubini Theorem. On the other side $|A||B|=|A'||B'|$, and since this holds for every $A',B'\in\mathcal{B}([0,1])$, this implies that $T$ is strongly mixing, which is a contradiction. 
\end{proof}
\noindent
Therefore we can define $S_k=T_k\times T_k$ where $\lbrace T_k\rbrace$ is the family defined by Chacon (section \ref{Ss:chacon}), and $S=\lim_{k\to\infty}S_k=T\times T$, where $T$ is the Canonical Chacon's map. \\

\noindent We show now that each $S_k$ can be decomposed into a fixed number of movements (as done in the first construction), each one arising as the action of a $BV$ divergence-free vector field. 
We start with $S_1$ to fix the notation and the notion of movements. We recall that by the previous analysis the map $T_1$ can be written in the language of permutations as
\begin{equation*}
    T_1\llcorner_{[0,1]\setminus R_1}=\left(\begin{matrix}I_{0,1}(1) & I_{0,1}(2) & I_{0,1}(3) & S_0 \\ I_{0,1}(2) & S_0 & I_{0,1}(1) & I_{0,1}(3)\end{matrix}\right).
\end{equation*}
For simplicity, if we associate $I_{0,1}(j)\rightarrow j$ and $S_0\rightarrow 4$ we write it as
\begin{equation}\label{notation_permutation}
    T_1\llcorner_{[0,1]\setminus R_1}=\left(\begin{matrix}1 & 2 & 3 & 4 \\ 2 & 4 & 1 & 3\end{matrix}\right).
\end{equation}
We represent the action of the map $S_1$ in the following matrix form, where the couples $\lbrace i,j\rbrace$,  $i,j\in\lbrace{1,2,3,4}\rbrace$ where $i,j$ represent respectively the row and the column index, denote the subsquares of $\mathbb{T}^2$. Finally, $c_s$ and $c_f$ are the \emph{starting configuration} and the \emph{final configuration}: 
\begin{equation}\label{configurations}
    c_s=\left(\begin{matrix}4,1 & 4,2 & 4,3 & 4,4 \\ 3,1 & 3,2 & 3,3 & 3,4 \\ 2,1 & 2,2 & 2,3 & 2,4 \\ 1,1 & 1,2 & 1,3 & 1,4
    \end{matrix}\right)\stackrel{S_1}{\longrightarrow}  c_f=\left(\begin{matrix}2,3 & 2,1 & 2,4 & 2,2 \\ 4,3 & 4,1 & 4,4 & 4,2 \\ 1,3 & 1,1 & 1,4 & 1,2 \\ 3,3 & 3,1 & 3,4 & 3,2
    \end{matrix}\right)
\end{equation}
For example, $(1,1)$ denotes the subsquare $I_{0,1}^2=[0,\frac{2}{9}]^2$, therefore the action of the map $S_1$ is $S_1(1,1)=(T_1(1),T_1(1))=(2,2)=I_{0,1}(2)^2=[\frac{2}{9},\frac{4}{9}]$, that is the subsquare represented by $(1,1)$ is sent in the position of the subsquare $(2,2)$. One can easily observe that  each row is sent into another row, with permuted column indexes (ex. the row $(\begin{matrix}2,1 & 2,2 & 2,3 & 2,4\end{matrix})$ is sent into the row $(\begin{matrix} 4,2 & 4,4 & 4,1 & 4,3\end{matrix})$). The same for columns: each column is sent into another column with permuted row indexes. \\

\noindent
Given the starting configuration $c_s$ and the final configuration $c_f$ \ref{configurations} we describe the movements allowed to pass from $c_s\rightarrow c_f$.
Then we have
\begin{equation}\label{eq_movements_1}
     \gamma_f=(\rho_c(4)\circ\rho_c(1)\circ e_c(1,2)\circ s^3_c\circ e_c(1,2))\circ(\rho_r(4)\circ\rho_r(1)\circ e_r(1,2)\circ s^3_r\circ e_r(1,2))(\gamma_s).
\end{equation}
See in the appendix the proof of this fact. 
\begin{proposition}
Let us fix $n\in\N$ and let us consider the map $S_n$. Let $\gamma_s,\gamma_f$ be the starting and final configurations for $S_n$. Then
\begin{equation}\label{eq_movements}
    \gamma_f=(\rho_c(h_n)\circ\rho_c(1)\circ e_c(1,2)\circ s^3_c\circ e_c(h_{n}-3,h_n-2))\circ(\rho_r(h_n)\circ\rho_r(1)\circ e_r(1,2)\circ s^3_r\circ e_r(h_{n}-3,h_{n}-2))(\gamma_s)
\end{equation}
\begin{remark}
We observe that the \eqref{eq_movements} is consistent with \eqref{eq_movements_1} since $h_1=4$.
\end{remark}
\begin{proof}
We write the map $T_n$ as a permutation according to the notation \eqref{notation_permutation} (controlla se deve essere $h_n$ o $h_{n+1}$, la notazione delle configurazioni non va bene!!).
\begin{equation}\label{notation_permutations_n}
    T_n\llcorner_{[0,1]\setminus R_n}=\left(\begin{matrix}1 & 2 & 3 & \dots & i & \dots & h_{n}-3 & h_n-2 & h_n-1 & h_n \\ 4 & 5 & 6  & \dots & i+3 & \dots & 2  & h_n & 1 & 3  \end{matrix}\right).
\end{equation}
The starting configuration $\gamma_s$ for $S_n$ is $\gamma_s=(r(1),r(2),\dots,r(h_n))$, while the final one is $\gamma_f=(r(h_n-1), r(h_n-3), r(h_n), r(1), r(2),\dots, r(h_n-4), r(h_n-2))$, and the same if we write the configuration by columns. If we apply $(\rho_r(h_n)\circ\rho_r(1)\circ e_r(1,2)\circ s^3_r\circ e_r(h_{n}-3,h_{n}-2))$ to $\gamma_s$ we find
\begin{itemize}
\item
$e_r(h_{n}-3,h_{n}-2)(r(1),r(2),\dots,r(h_n))=(r(1),r(2),\dots,r(h_n-4), \bar{r}(h_n-2), \bar{r}(h_n-3), r(h_n-1), r(h_n))$,
    \item
    $s^3_r(r(1),r(2),\dots,r(h_n-4), \bar{r}(h_n-2), \bar{r}(h_n-3), r(h_n-1), r(h_n))= (\bar{r}(h_n-3), r(h_n-1), r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))$,
    \item $e_r(1,2)(\bar{r}(h_n-3), r(h_n-1), r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))=(\bar{r}(h_n-1),r(h_n-3),r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))$,
    \item $\rho_r(h_n)\circ\rho_r(1)(\bar{r}(h_n-1),r(h_n-3),r(h_n), r(1), r(2),\dots, r(h_n-4), \bar{r}(h_n-2))=(r(h_n-1),r(h_n-3),r(h_n),r(1),r(2),\dots)=\gamma_m$.
\end{itemize}
After this first set of movements we have the rows in the correct position, while the columns are ordered as $(c(1),c(2),\dots, c(h_n))$. This set of movements (horizontal/vertical ones) does not change the order of columns, as the second set of movements doesn't change the order of rows (questo è importante ma devo scriverlo in modo più esplicito). So applying the second set of movements to $\gamma_m$ since the order of rows does not change, while for columns we have the correct new order we finally get $\gamma_f$. Sono d'accordo che sia detto abbastanza a cazzo.
\end{proof}
 \end{proposition}
 \noindent The previous proposition shows that the number of movements to recover the final configuration of each map $S_n$ from the starting one is fixed: this result allows us to construct vector fields associated to each $S_n$. Anche le $S_n$ sono cicliche? da chiarirtelo.

%\noindent We underline that the choice of presenting two examples with different approaches relies on the fact that the first example, which is the most natural once knowing Chacon's example, does not work in the unit square, since it heavily exploits the structure of the torus for having good compactness estimates on the vector fields. The second example instead is less flexible but it furnishes a weakly mixing vector field on the unit square. \\

 \begin{theorem}\label{product}
    Let $T\in G(\mathbb{T}^2)$ be an automorphism. Then $T$ is weakly mixing iff $T\times T$ is weakly mixing.
    \end{theorem}
    {\color{red}\begin{remark}
    Does it hold $T$ w.m. iff $T\times \dots\times T$ w.m.?
    \end{remark}}
    
    \begin{definition}[Exchange rows vector field]
Let $\gamma\in\mathcal{C}(k)$ be a configuration. Let $r(i)$, $r(i')$ with $i\leq i'$ be two rows.  The exchange rows \emph{vector field} is a vector field $b^{E_r}(t)(i,i')\in L^\infty_t\BV_x$   such that, if $X^{E_r}(i,i')$ is its RLF evaluated at time $t=1$ then 
 \begin{equation}
     X^{E_r}(i,i')(\T^2)=E_r(i,i')(\gamma),\quad\forall\gamma\in\mathcal{C}(k).
 \end{equation}
 \end{definition}
\begin{remark}
Analogously, given a configuration $\gamma\in\mathcal{C}(k)$ and two columns $c(j),c(j')$ with $j\leq j'$ one can define the Exchange columns vector field $b^{E_c}(t)(j,j')$.
\end{remark}

\noindent
The construction of the Exchange rows (columns) vector fields exploit always rotations. More precisely, let us fix  $\gamma\in\mathcal{C}(k)$ and two rows $r(i)$, $r(i')$ with $i\leq i'$.
Then consider the subrectangle $Q(i,i')=\cup_{l=i}^j H_l$. Define the following flow
\begin{equation*}
   X^{E_r}(t)(i,i')=
   \begin{cases}
   \chi^{-1}\circ r_{4t}\circ \chi & x\in \mathring{Q(i,i')}, \ t\in\left[0,\frac{1}{2}\right], \\
		\chi_{Q_{lj}}^{-1}\circ r_{4t}\circ \chi_{Q_{lj}} & x\in\mathring{Q_{lj}},  t\in\left[\frac{1}{2},1\right], \forall l\in\lbrace i,i+1,\dots,i'\rbrace,\forall j \\
		x & \text{otherwise},
   \end{cases}
\end{equation*}
where $\chi$ is the affine map sending $Q(i,i')$ into $\T^2$ and $\chi_{Q_{lj}}$ is the affine map sending $Q_{lj}$ into $\T^2$.
Then, defining always $b^{E_r}(t)$ as in \ref{vect:field:ass}, always using Lemma \ref{rot:flow:square}, one can check that, for every $t\in[0,1]$, \begin{equation}
    \TV(b^{E_r}(t))(\T^2)\leq 4\cdot 4\left(1+\left(\frac{i'-i+1}{k}\right)^2\right).
\end{equation}
\begin{example}
In Figure \ref{fig:exchangerowsvf} an explicit and visual example of the action of the vector field $b(t)^{E_r}(1,3)$ on the torus (compare with Example \ref{ex:exchange:rows}).
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{exchangerowsvf.png}
    \caption{Action of the Exchange rows vector field $b(t)^{E_r}(1,3)$.}
    \label{fig:exchangerowsvf}
\end{figure}
\end{example}
\begin{definition}[Exchange]
Let $\gamma\in\mathcal{C}(n)$ as above. Let $r(i)$, $r(i')$ with $i\leq i'$ two rows and $c(j),c(j')$ with $j\leq j'$ two columns. Then an \emph{exchange} of rows $E_r(i,i'):\mathcal{C}(n)\rightarrow \mathcal{C}(n)$ is the following configuration
\begin{equation}
    E_r(i,i')(\gamma)=(r(1),r(2),\dots, r(i-1), \bar{r}(i'),\bar{r}(i'-1),\dots,\bar{r}(i+1),\bar{r}(i), r(i'+1),\dots, r(n))^T,
\end{equation}
while an exchange of columns $E_c(j,j'):\mathcal{C}(n)\rightarrow \mathcal{C}(n)$ is the following configuration
\begin{equation}
    E_c(j,j')(\gamma)=(c(1),c(2),\dots, c(j-1), \bar{c}(j'),\bar{c}(j'-1),\dots,\bar{c}(j+1),\bar{c}(j), c(j'+1),\dots, c(n)).
\end{equation}
We will denote by $E_r(i)=E_r(i,i)$ and $E_c(j)=E_c(j,j)$.
\end{definition}
\begin{example}\label{ex:exchange:rows}
We give the example of some configuration $\gamma$ and the new configuration $E_r(1,3)(\gamma)$ obtained by exchanging rows:\begin{equation*}
    \gamma=\left(\begin{matrix}1 & 2 & 3 & 4 \\ 5 & 6 & 7 & 8 \\ 9 & 10 & 11 & 12 \\ 13 & 14 & 15 & 16
    \end{matrix}\right) \qquad
    E_r(1,3)(\gamma)=\left(\begin{matrix}12 & 11 & 10 & 9 \\ 8 & 7 & 6 & 5 \\ 4 & 3 & 2 & 1 \\ 13 & 14 & 15 & 16
    \end{matrix}\right).
    \end{equation*}
\end{example}
\begin{definition}\label{def_reversed}
Let $r(i)=\begin{matrix}(i,j_1 & i,j_2 & \dots  & i,j_n)\end{matrix}$ be a row of length $n$. Then we denote by \begin{equation}\bar{r}(i)=\begin{matrix}(i,j_n & i,j_{n-1} & \dots  & i,j_1)\end{matrix}\end{equation} the \emph{reversed row}.
\end{definition}
\begin{remark}
We can define similarly the reversed column $\bar{c}(j)$.
\end{remark}
